Exploring ChatGPT for Face Presentation Attack Detection in Zero and Few-Shot in-Context Learning

This study highlights the potential of ChatGPT (specifically GPT-4o) as a competitive alternative for Face Presentation Attack Detection (PAD), outperforming several PAD models, including commercial solutions, in specific scenarios. Our results show that GPT-4o demonstrates high consistency, particularly in few-shot in-context learning, where its performance improves as more examples are provided (reference data). We also observe that detailed prompts enable the model to provide scores reliably, a behavior not observed with concise prompts. Additionally, explanation-seeking prompts slightly enhance the model's performance by improving its interpretability. Remarkably, the model exhibits emergent reasoning capabilities, correctly predicting the attack type (print or replay) with high accuracy in few-shot scenarios, despite not being explicitly instructed to classify attack types. Despite these strengths, GPT-4o faces challenges in zero-shot tasks, where its performance is limited compared to specialized PAD systems. Experiments were conducted on a subset of the SOTERIA dataset, ensuring compliance with data privacy regulations by using only data from consenting individuals. These findings underscore GPT-4o's promise in PAD applications, laying the groundwork for future research to address broader data privacy concerns and improve cross-dataset generalization. Code available here: https://gitlab.idiap.ch/bob/bob.paper.wacv2025_chatgpt_face_pad

==> Makefile <==
TEXFILE=PaperForReview.tex

PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex
	pdflatex $(@:%.pdf=%.tex); \
	bibtex $(@:%.pdf=%); \
	pdflatex $(@:%.pdf=%.tex); \
	pdflatex $(@:%.pdf=%.tex);

all: $(PDFFILE)

clean:
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.blg
	@rm -vf *.aux *.glo *.dvi *.ps *.out *.brf *.bbl $(PDFFILE)



==> graphics/diagram.tex <==

\begin{tikzpicture}[
    box/.style={rectangle, draw, text width=4cm, text centered, rounded corners, minimum height=2cm, font=\huge},
    emptybox/.style={rectangle, draw=none, pattern=north east lines, text width=4cm, text centered, minimum height=2cm, font=\huge},
    rowlabel/.style={anchor=east, text width=2cm, text centered, font=\huge},
    columnlabel/.style={anchor=south, text width=4cm, text centered, font=\huge}
]

% Column labels
\node[columnlabel] (system) at (2, 6) {System};
\node[columnlabel] (user1) at (7, 6) {User};
\node[columnlabel] (user2) at (12, 6) {User};

% Row labels
\node[rowlabel] (row1) at (0, 4.5) {zero-shot};
\node[rowlabel] (row2) at (0, 1) {few-shot};

% System column
\node[box, fill=blue!20] (sys1) at (2, 4.5) {Role description};
\node[box, fill=blue!20] (sys2) at (2, 1) {Role description};

% User 1 column
\node[emptybox] (user1_1) at (7, 4.5) {N/A};
\node[box, fill=yellow!20] (user1_2) at (7, 1) {Reference image \\ + Text description};

% User 2 column
\node[box, fill=red!20] (user2_1) at (12, 4.5) {Probe image \\ + Task to be performed};
\node[box, fill=red!20] (user2_2) at (12, 1) {Probe image \\ + Task to be performed};

% % Draw horizontal separators
% \draw[dashed] (-0.5, 4) -- (14, 4);

% % Draw vertical separators
% \draw[dashed] (4.5, 7) -- (4.5, 2);

\end{tikzpicture}


